Variable elimination for building interpreters

In this paper, we build an interpreter by reusing host language functions instead of recoding mechanisms of function application that are already available in the host language (the language which is used to build the interpreter). In order to transform user-defined functions into host language functions we use combinatory logic : lambda-abstractions are transformed into a composition of combinators. We provide a mechanically checked proof that this step is correct for the call-by-value strategy with imperative features.

==> mabibmodif.tex <==


\newcommand{\etalchar}[1]{$^{#1}$}
\begin{thebibliography}{RBCL{\etalchar{+}}06}

\bibitem[COQ]{coq}
{The Coq Proof Assistant}.
\newblock Web site : \url{http://coq.inria.fr}.

\bibitem[OCaml]{caml_site}
Objective {C}aml.
\newblock Web site : \url{http://caml.inria.fr/ocaml/}.
\end{thebibliography}


\begin{thebibliography*}{RBCL{\etalchar{+}}06}


\bibitem[Bar06]{Barzilay2006}
Eli Barzilay.
\newblock A self-hosting evaluator using {HOAS} -- a \nom{Scheme} pearl.
\newblock In {\em Scheme and Functional Programming Workshop, University of
  Chicago Technical Report TR-2006-06}, 2006.

\bibitem[CF58]{combinatory-logic}
Haskell~B. Curry and Robert Feys.
\newblock {\em Combinatory Logic}, volume~I.
\newblock North Holland, 1958.

\bibitem[CH06]{history_of_lambda_calculus}
Felice Cardone and J.~Roger Hindley.
\newblock History of lambda-calculus and combinatory logic.
\newblock Research Report MRRS-05-06, Swansea University Mathematics
  Department, 2006.

\bibitem[Coh04]{these-Julien}
Julien Cohen.
\newblock {\em Int\'egration des collections topologiques et des
  transformations dans un langage fonctionnel}.
\newblock PhD thesis, universit\'e d'\'Evry Val d'Essonne, December 2004.


\bibitem[Dil02]{diller02}
Antoni Diller.
\newblock Efficient multi-variate abstraction using an array representation for
  combinators.
\newblock {\em Inf. Process. Lett.}, 84(6):311--317, 2002.

\bibitem[GD92]{cbv-combinatory-logic}
John Gateley and Bruce~F. Duba.
\newblock Call-by-value combinatory logic and the lambda-value calculus.
\newblock In {\em Mathematical Foundations of Programming Semantics, 7th
  International Conference, 1991}, volume 598 of {\em Lecture Notes in Computer
  Science}, pages 41--53. Springer, 1992.

\bibitem[HD97]{thunks}
John Hatcliff and Olivier Danvy.
\newblock Thunks and the $\lambda$-calculus.
\newblock {\em Journal of Functional Programming}, 7(3):303--319, 1997.


\bibitem[PE88]{HOAS}
F.~Pfenning and C.~Elliot.
\newblock Higher-order abstract syntax.
\newblock In {\em Proceedings of the ACM SIGPLAN 1988 conference on Programming
  Language design and Implementation}, pages 199--208. ACM Press, 1988.

\bibitem[PJW93]{monades93}
Simon~L. Peyton~Jones and Philip Wadler.
\newblock Imperative functional programming.
\newblock In {\em POPL '93: Proceedings of the 20th ACM SIGPLAN-SIGACT
  symposium on Principles of programming languages}, pages 71--84, New York,
  NY, USA, 1993. ACM.

\bibitem[Plo75]{plotkin}
Gordon Plotkin.
\newblock Call-by-name, call-by-value and the $\lambda$-calculus.
\newblock {\em Theoretical Computer Science}, 1:125--159, 1975.

\bibitem[RBCL{\etalchar{+}}06]{godin2006}
Pierre Barbier~de Reuille, Isabelle Bohn-Courseau, Karin Ljung, Halima Morin,
  Nicola Carraro, Christophe Godin, and Jan Traas.
\newblock Computer simulations reveal properties of the cell-cell signaling
  network at the shoot apex in {A}rabidopsis.
\newblock {\em Proceedings of the National Academy of Sciences},
  103(5):1627--1632, 2006.

\bibitem[WW03]{boxes-go-bananas}
Geoffrey Washburn and Stephanie Weirich.
\newblock Boxes go bananas: Encoding higher-order abstract syntax with
  parametric polymorphism.
\newblock In {\em ACM SIGPLAN International Conference on Functional
  Programming (ICFP)}, pages 249--262, 2003.

\end{thebibliography*}

